DiagESC: Dialogue Synthesis for Integrating Depression Diagnosis into Emotional Support Conversation

Dialogue systems for mental health care aim to provide appropriate support to individuals experiencing mental distress. While extensive research has been conducted to deliver adequate emotional support, existing studies cannot identify individuals who require professional medical intervention and cannot offer suitable guidance. We introduce the Diagnostic Emotional Support Conversation task for an advanced mental health management system. We develop the DESC dataset to assess depression symptoms while maintaining user experience by utilizing task-specific utterance generation prompts and a strict filtering algorithm. Evaluations by professional psychological counselors indicate that DESC has a superior ability to diagnose depression than existing data. Additionally, conversational quality evaluation reveals that DESC maintains fluent, consistent, and coherent dialogues.

==> custom.tex <==
% Use this file for citations not found in the ACL Anthology (contained in "anthology.bib").

@book{Aho:72,
    author  = {Alfred V. Aho and Jeffrey D. Ullman},
    title   = {The Theory of Parsing, Translation and Compiling},
    year    = "1972",
    volume  = "1",
    publisher = {Prentice-Hall},
    address = {Englewood Cliffs, NJ}
}

@book{APA:83,
    author  = {{American Psychological Association}},
    title   = {Publications Manual},
    year    = "1983",
    publisher = {American Psychological Association},
    address = {Washington, DC}
}

@article{Chandra:81,
	author = {Ashok K. Chandra and Dexter C. Kozen and Larry J. Stockmeyer},
	year = "1981",
	title = {Alternation},
	journal = {Journal of the Association for Computing Machinery},
	volume = "28",
	number = "1",
	pages = "114--133",
	doi = "10.1145/322234.322243",
}

@inproceedings{andrew2007scalable,
  title={Scalable training of {L1}-regularized log-linear models},
  author={Andrew, Galen and Gao, Jianfeng},
  booktitle={Proceedings of the 24th International Conference on Machine Learning},
  pages={33--40},
  year={2007},
}

@book{Gusfield:97,
    author  = {Dan Gusfield},
    title   = {Algorithms on Strings, Trees and Sequences},
    year    = "1997",
    publisher = {Cambridge University Press},
    address = {Cambridge, UK}
}

@article{rasooli-tetrault-2015,
    author    = {Mohammad Sadegh Rasooli and Joel R. Tetreault},
    title     = {Yara Parser: {A} Fast and Accurate Dependency Parser},
    journal   = {Computing Research Repository},
    volume    = {arXiv:1503.06733},
    year      = {2015},
    url       = {http://arxiv.org/abs/1503.06733},
    note    = {version 2}
}

@article{Ando2005,
	Acmid = {1194905},
	Author = {Ando, Rie Kubota and Zhang, Tong},
	Issn = {1532-4435},
	Issue_Date = {12/1/2005},
	Journal = {Journal of Machine Learning Research},
	Month = dec,
	Numpages = {37},
	Pages = {1817--1853},
	Publisher = {JMLR.org},
	Title = {A Framework for Learning Predictive Structures from Multiple Tasks and Unlabeled Data},
	Volume = {6},
	Year = {2005}
}

@article{LIM2022334,
    title = {Chatbot-Delivered Psychotherapy for Adults With Depressive and Anxiety Symptoms: A Systematic Review and Meta-Regression},
    journal = {Behavior Therapy},
    volume = {53},
    number = {2},
    pages = {334-347},
    year = {2022},
    issn = {0005-7894},
    doi = {https://doi.org/10.1016/j.beth.2021.09.007},
    url = {https://www.sciencedirect.com/science/article/pii/S0005789421001258},
    author = {Shi Min Lim and Chyi Wey Claudine Shiau and Ling Jie Cheng and Ying Lau},
    keywords = {artificial intelligence, psychotherapy, depression, meta-analysis, systematic review},
    abstract = {Although psychotherapy is a well-established treatment for depression and anxiety, chatbot-delivered psychotherapy is an emerging field that has yet to be explored in depth. This review aims to (a) examine the effectiveness of chatbot-delivered psychotherapy in improving depressive symptoms among adults with depression or anxiety, and (b) evaluate the preferred features for the design of chatbot-delivered psychotherapy. Eight electronic databases were searched for relevant randomized controlled trials. Meta-analysis and random effects meta-regression was conducted using Comprehensive Meta-Analysis 3.0 software. Overall effect was measured using Hedges’s g and determined using z statistics at significance level p < .05. Assessment of heterogeneity was done using χ2 and I2 tests. A meta-analysis of 11 trials revealed that chatbot-delivered psychotherapy significantly improved depressive symptoms (g = 0.54, 95% confidence interval [−0.66, −0.42], p < .001). Although no significant subgroup differences were detected, results revealed larger effect sizes for samples of clinically diagnosed anxiety or depression, chatbots with an embodiment, a combination of types of input and output formats, less than 10 sessions, problem-solving therapy, off-line platforms, and in different regions of the United States than their counterparts. Meta-regression did not identify significant covariates that had an impact on depressive symptoms. Chatbot-delivered psychotherapy can be adopted in health care institutions as an alternative treatment for depression and anxiety. More high-quality trials are warranted to confirm the effectiveness of chatbot-delivered psychotherapy on depressive symptoms. PROSPERO registration number: CRD42020153332.}
}

@inproceedings{li2017dailydialog,
  title={DailyDialog: A Manually Labelled Multi-turn Dialogue Dataset},
  author={Li, Yanran and Su, Hui and Shen, Xiaoyu and Li, Wenjie and Cao, Ziqiang and Niu, Shuzi},
  booktitle={Proceedings of the Eighth International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  pages={986--995},
  year={2017}
}

@inproceedings{chen2018emotionlines,
  title={EmotionLines: An Emotion Corpus of Multi-Party Conversations},
  author={Hsu, Chao-Chun and Chen, Sheng-Yeh and Kuo, Chuan-Chun and Huang, Ting-Hao and Ku, Lun-Wei},
  booktitle={Proceedings of the Eleventh International Conference on Language Resources and Evaluation (LREC 2018)},
  year={2018}
}

@inproceedings{chatterjee2019semeval,
  title={SemEval-2019 task 3: EmoContext contextual emotion detection in text},
  author={Chatterjee, Ankush and Narahari, Kedhar Nath and Joshi, Meghana and Agrawal, Puneet},
  booktitle={Proceedings of the 13th international workshop on semantic evaluation},
  pages={39--48},
  year={2019}
}

@ARTICLE{8649596,
  author={Lubis, Nurul and Sakti, Sakriani and Yoshino, Koichiro and Nakamura, Satoshi},
  journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
  title={Positive Emotion Elicitation in Chat-Based Dialogue Systems}, 
  year={2019},
  volume={27},
  number={4},
  pages={866-877},
  keywords={Neural networks;Databases;Speech processing;Appraisal;Affective computing;Emotion recognition;Crowdsourcing;Natural language processing;emotion elicitation;affective computing;chat-based dialogue system;neural networks},
  doi={10.1109/TASLP.2019.2900910}}

@inproceedings{rashkin2019towards,
  title={Towards Empathetic Open-domain Conversation Models: A New Benchmark and Dataset},
  author={Rashkin, Hannah and Smith, Eric Michael and Li, Margaret and Boureau, Y-Lan},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={5370--5381},
  year={2019}
}

@inproceedings{liu2021towards,
  title={Towards Emotional Support Dialog Systems},
  author={Liu, Siyang and Zheng, Chujie and Demasi, Orianna and Sabour, Sahand and Li, Yu and Yu, Zhou and Jiang, Yong and Huang, Minlie},
  booktitle={Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  pages={3469--3483},
  year={2021}
}

@book{Hill2009,
  author    = {Clara E. Hill},
  title     = {Helping Skills: Facilitating, Exploration, Insight, and Action},
  year      = {2009},
  edition   = {3},
  publisher = {American Psychological Association},
}

@inproceedings{ide2021multi,
  title={Multi-Task Learning of Generation and Classification for Emotion-Aware Dialogue Response Generation},
  author={Ide, Tatsuya and Kawahara, Daisuke},
  booktitle={Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Student Research Workshop},
  pages={119--125},
  year={2021}
}

@inproceedings{wei2019emotion,
  title={Emotion-aware chat machine: Automatic emotional response generation for human-like emotional interaction},
  author={Wei, Wei and Liu, Jiayi and Mao, Xianling and Guo, Guibing and Zhu, Feida and Zhou, Pan and Hu, Yuchong},
  booktitle={Proceedings of the 28th ACM international conference on information and knowledge management},
  pages={1401--1410},
  year={2019}
}

@inproceedings{zandie2020emptransfo,
  title={Emptransfo: A multi-head transformer architecture for creating empathetic dialog systems},
  author={Zandie, Rohola and Mahoor, Mohammad H},
  booktitle={The thirty-third international flairs conference},
  year={2020}
}

@inproceedings{ghosal2020cosmic,
  title={COSMIC: COmmonSense knowledge for eMotion Identification in Conversations},
  author={Ghosal, Deepanway and Majumder, Navonil and Gelbukh, Alexander and Mihalcea, Rada and Poria, Soujanya},
  booktitle={Findings of the Association for Computational Linguistics: EMNLP 2020},
  pages={2470--2481},
  year={2020}
}

@inproceedings{majumder2020mime,
  title={MIME: MIMicking Emotions for Empathetic Response Generation},
  author={Majumder, Navonil and Hong, Pengfei and Peng, Shanshan and Lu, Jiankun and Ghosal, Deepanway and Gelbukh, Alexander and Mihalcea, Rada and Poria, Soujanya},
  booktitle={Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  pages={8968--8979},
  year={2020}
}

@article{Li_Li_Ren_Ren_Chen_2022, title={Knowledge Bridging for Empathetic Dialogue Generation}, volume={36}, url={https://ojs.aaai.org/index.php/AAAI/article/view/21347}, DOI={10.1609/aaai.v36i10.21347}, abstractNote={Lack of external knowledge makes empathetic dialogue systems difficult to perceive implicit emotions and learn emotional interactions from limited dialogue history. To address the above problems, we propose to leverage external knowledge, including commonsense knowledge and emotional lexical knowledge, to explicitly understand and express emotions in empathetic dialogue generation. We first enrich the dialogue history by jointly interacting with external knowledge and construct an emotional context graph. Then we learn emotional context representations from the knowledge-enriched emotional context graph and distill emotional signals, which are the prerequisites to predicate emotions expressed in responses. Finally, to generate the empathetic response, we propose an emotional cross-attention mechanism to learn the emotional dependencies from the emotional context graph. Extensive experiments conducted on a benchmark dataset verify the effectiveness of the proposed method. In addition, we find the performance of our method can be further improved by integrating with a pre-trained model that works orthogonally.}, number={10}, journal={Proceedings of the AAAI Conference on Artificial Intelligence}, author={Li, Qintong and Li, Piji and Ren, Zhaochun and Ren, Pengjie and Chen, Zhumin}, year={2022}, month={Jun.}, pages={10993-11001} }

@inproceedings{cheng2023pal,
  title={PAL: Persona-Augmented Emotional Support Conversation Generation},
  author={Cheng, Jiale and Sabour, Sahand and Sun, Hao and Chen, Zhuang and Huang, Minlie},
  booktitle={Findings of the Association for Computational Linguistics: ACL 2023},
  pages={535--554},
  year={2023}
}

@inproceedings{deshpande2017depression,
  title={Depression detection using emotion artificial intelligence},
  author={Deshpande, Mandar and Rao, Vignesh},
  booktitle={2017 international conference on intelligent sustainable systems (iciss)},
  pages={858--862},
  year={2017},
  organization={IEEE}
}

@inproceedings{orabi2018deep,
  title={Deep learning for depression detection of twitter users},
  author={Orabi, Ahmed Husseini and Buddhitha, Prasadith and Orabi, Mahmoud Husseini and Inkpen, Diana},
  booktitle={Proceedings of the fifth workshop on computational linguistics and clinical psychology: from keyboard to clinic},
  pages={88--97},
  year={2018}
}

@article{kroenke2009phq,
  title={The PHQ-8 as a measure of current depression in the general population},
  author={Kroenke, Kurt and Strine, Tara W and Spitzer, Robert L and Williams, Janet BW and Berry, Joyce T and Mokdad, Ali H},
  journal={Journal of affective disorders},
  volume={114},
  number={1-3},
  pages={163--173},
  year={2009},
  publisher={Elsevier}
}

@inproceedings{ringeval2019avec,
  title={AVEC 2019 workshop and challenge: state-of-mind, detecting depression with AI, and cross-cultural affect recognition},
  author={Ringeval, Fabien and Schuller, Bj{\"o}rn and Valstar, Michel and Cummins, Nicholas and Cowie, Roddy and Tavabi, Leili and Schmitt, Maximilian and Alisamir, Sina and Amiriparian, Shahin and Messner, Eva-Maria and others},
  booktitle={Proceedings of the 9th International on Audio/visual Emotion Challenge and Workshop},
  pages={3--12},
  year={2019}
}

@inproceedings{gratch2014distress,
  title={The distress analysis interview corpus of human and computer interviews.},
  author={Gratch, Jonathan and Artstein, Ron and Lucas, Gale M and Stratou, Giota and Scherer, Stefan and Nazarian, Angela and Wood, Rachel and Boberg, Jill and DeVault, David and Marsella, Stacy and others},
  booktitle={LREC},
  pages={3123--3128},
  year={2014},
  organization={Reykjavik}
}

@inproceedings{kulkarni-etal-2024-synthdst,
    title = "{S}ynth{DST}: Synthetic Data is All You Need for Few-Shot Dialog State Tracking",
    author = "Kulkarni, Atharva  and
      Tseng, Bo-Hsiang  and
      Moniz, Joel  and
      Piraviperumal, Dhivya  and
      Yu, Hong  and
      Bhargava, Shruti",
    editor = "Graham, Yvette  and
      Purver, Matthew",
    booktitle = "Proceedings of the 18th Conference of the European Chapter of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = mar,
    year = "2024",
    address = "St. Julian{'}s, Malta",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2024.eacl-long.120",
    pages = "1988--2001",
    abstract = "In-context learning with Large Language Models (LLMs) has emerged as a promising avenue of research in Dialog State Tracking (DST). However, the best-performing in-context learning methods involve retrieving and adding similar examples to the prompt, requiring access to labeled training data. Procuring such training data for a wide range of domains and applications is time-consuming, expensive, and, at times, infeasible. While zero-shot learning requires no training data, it significantly lags behind the few-shot setup. Thus, {`}\textit{Can we efficiently generate synthetic data for any dialogue schema to enable few-shot prompting?}' Addressing this question, we propose , a data generation framework tailored for DST, utilizing LLMs. Our approach only requires the dialogue schema and a few hand-crafted dialogue templates to synthesize natural, coherent, and free-flowing dialogues with DST annotations. Few-shot learning using data from results in $4-5\%$ improvement in Joint Goal Accuracy over the zero-shot baseline on MultiWOZ 2.1 and 2.4. Remarkably, our few-shot learning approach recovers nearly 98{\%} of the performance compared to the few-shot setup using human-annotated training data.",
}

@inproceedings{kim2023soda,
  title={SODA: Million-scale Dialogue Distillation with Social Commonsense Contextualization},
  author={Kim, Hyunwoo and Hessel, Jack and Jiang, Liwei and West, Peter and Lu, Ximing and Yu, Youngjae and Zhou, Pei and Le Bras, Ronan and Alikhani, Malihe and Kim, Gunhee and others},
  booktitle={The 2023 Conference on Empirical Methods in Natural Language Processing},
  year={2023}
}

@inproceedings{bao-etal-2023-synthetic,
    title = "A Synthetic Data Generation Framework for Grounded Dialogues",
    author = "Bao, Jianzhu  and
      Wang, Rui  and
      Wang, Yasheng  and
      Sun, Aixin  and
      Li, Yitong  and
      Mi, Fei  and
      Xu, Ruifeng",
    editor = "Rogers, Anna  and
      Boyd-Graber, Jordan  and
      Okazaki, Naoaki",
    booktitle = "Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2023",
    address = "Toronto, Canada",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2023.acl-long.608",
    doi = "10.18653/v1/2023.acl-long.608",
    pages = "10866--10882",
    abstract = "Training grounded response generation models often requires a large collection of grounded dialogues. However, it is costly to build such dialogues. In this paper, we present a synthetic data generation framework (SynDG) for grounded dialogues. The generation process utilizes large pre-trained language models and freely available knowledge data (e.g., Wikipedia pages, persona profiles, etc.). The key idea of designing SynDG is to consider dialogue flow and coherence in the generation process. Specifically, given knowledge data, we first heuristically determine a dialogue flow, which is a series of knowledge pieces. Then, we employ T5 to incrementally turn the dialogue flow into a dialogue. To ensure coherence of both the dialogue flow and the synthetic dialogue, we design a two-level filtering strategy, at the flow-level and the utterance-level respectively. Experiments on two public benchmarks show that the synthetic grounded dialogue data produced by our framework is able to significantly boost model performance in both full training data and low-resource scenarios.",
}

@inproceedings{kim2024kocosa,
  title={KoCoSa: Korean Context-aware Sarcasm Detection Dataset},
  author={Kim, Yumin and Suh, Heejae and Kim, Mingi and Won, Dongyeon and Lee, Hwanhee},
  booktitle={Proceedings of the 2024 Joint International Conference on Computational Linguistics, Language Resources and Evaluation (LREC-COLING 2024)},
  pages={9890--9904},
  year={2024}
}

@article{li2024stylechat,
  title={StyleChat: Learning Recitation-Augmented Memory in LLMs for Stylized Dialogue Generation},
  author={Li, Jinpeng and Zhang, Zekai and Tu, Quan and Cheng, Xin and Zhao, Dongyan and Yan, Rui},
  journal={arXiv preprint arXiv:2403.11439},
  year={2024}
}

@article{ding2024data,
  title={Data augmentation using llms: Data perspectives, learning paradigms and challenges},
  author={Ding, Bosheng and Qin, Chengwei and Zhao, Ruochen and Luo, Tianze and Li, Xinze and Chen, Guizhen and Xia, Wenhan and Hu, Junjie and Luu, Anh Tuan and Joty, Shafiq},
  journal={arXiv preprint arXiv:2403.02990},
  year={2024}
}

@inproceedings{lewis2017deal,
  title={Deal or No Deal? End-to-End Learning of Negotiation Dialogues},
  author={Lewis, Mike and Yarats, Denis and Dauphin, Yann and Parikh, Devi and Batra, Dhruv},
  booktitle={Proceedings of the 2017 Conference on Empirical Methods in Natural Language Processing},
  pages={2443--2453},
  year={2017}
}

@inproceedings{kenton2019bert,
  title={BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding},
  author={Kenton, Jacob Devlin Ming-Wei Chang and Toutanova, Lee Kristina},
  booktitle={Proceedings of NAACL-HLT},
  pages={4171--4186},
  year={2019}
}

@article{denecke2021artificial,
  title={Artificial intelligence for chatbots in mental health: opportunities and challenges},
  author={Denecke, Kerstin and Abd-Alrazaq, Alaa and Househ, Mowafa},
  journal={Multiple perspectives on artificial intelligence in healthcare: Opportunities and challenges},
  pages={115--128},
  year={2021},
  publisher={Springer}
}

@inproceedings{
    hu2022lora,
    title={Lo{RA}: Low-Rank Adaptation of Large Language Models},
    author={Edward J Hu and Yelong Shen and Phillip Wallis and Zeyuan Allen-Zhu and Yuanzhi Li and Shean Wang and Lu Wang and Weizhu Chen},
    booktitle={International Conference on Learning Representations},
    year={2022},
    url={https://openreview.net/forum?id=nZeVKeeFYf9}
}

@inproceedings{hou2018sequence,
  title={Sequence-to-Sequence Data Augmentation for Dialogue Language Understanding},
  author={Hou, Yutai and Liu, Yijia and Che, Wanxiang and Liu, Ting},
  booktitle={Proceedings of the 27th International Conference on Computational Linguistics},
  pages={1234--1245},
  year={2018}
}

@inproceedings{tang2019target,
  title={Target-Guided Open-Domain Conversation},
  author={Tang, Jianheng and Zhao, Tiancheng and Xiong, Chenyan and Liang, Xiaodan and Xing, Eric and Hu, Zhiting},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  year={2019},
  organization={Association for Computational Linguistics}
}

@article{kroenke2001phq,
  title={The PHQ-9: validity of a brief depression severity measure},
  author={Kroenke, Kurt and Spitzer, Robert L and Williams, Janet BW},
  journal={Journal of general internal medicine},
  volume={16},
  number={9},
  pages={606--613},
  year={2001},
  publisher={Wiley Online Library}
}

@article{wei2022chain,
  title={Chain-of-thought prompting elicits reasoning in large language models},
  author={Wei, Jason and Wang, Xuezhi and Schuurmans, Dale and Bosma, Maarten and Xia, Fei and Chi, Ed and Le, Quoc V and Zhou, Denny and others},
  journal={Advances in neural information processing systems},
  volume={35},
  pages={24824--24837},
  year={2022}
}

@article{cohen1968weighted,
  title={Weighted kappa: Nominal scale agreement provision for scaled disagreement or partial credit.},
  author={Cohen, Jacob},
  journal={Psychological bulletin},
  volume={70},
  number={4},
  pages={213},
  year={1968},
  publisher={American Psychological Association}
}

@INPROCEEDINGS{10045938,
  author={Chivinge, Lincoln and Nyandoro, Leslie Kudzai and Zvarevashe, Kudakwashe},
  booktitle={2022 1st Zimbabwe Conference of Information and Communication Technologies (ZCICT)}, 
  title={Quadratic Weighted Kappa Score Exploration in Diabetic Retinopathy Severity Classification Using EfficientNet}, 
  year={2022},
  volume={},
  number={},
  pages={1-9},
  keywords={Deep learning;Visualization;Sensitivity;Retinopathy;Pipelines;Medical services;Feature extraction;Diabetic Retinopathy Detection;Quadratic Weighted Kappa;Image Augmentation;Transfer Learning},
  doi={10.1109/ZCICT55726.2022.10045938}}

@inproceedings{nirthika2020loss,
  title={Loss functions for optimizing Kappa as the evaluation measure for classifying diabetic retinopathy and prostate cancer images},
  author={Nirthika, Rajendran and Manivannan, Siyamalan and Ramanan, Amirthalingam},
  booktitle={2020 IEEE 15th international conference on industrial and information systems (ICIIS)},
  pages={144--149},
  year={2020},
  organization={IEEE}
}

@article{haque2018measuring,
  title={Measuring depression symptom severity from spoken language and 3D facial expressions},
  author={Haque, Albert and Guo, Michelle and Miner, Adam S and Fei-Fei, Li},
  journal={arXiv preprint arXiv:1811.08592},
  year={2018}
}

@article{he2018automated,
  title={Automated depression analysis using convolutional neural networks from speech},
  author={He, Lang and Cao, Cui},
  journal={Journal of biomedical informatics},
  volume={83},
  pages={103--111},
  year={2018},
  publisher={Elsevier}
}

@article{low2020automated,
  title={Automated assessment of psychiatric disorders using speech: A systematic review},
  author={Low, Daniel M and Bentley, Kate H and Ghosh, Satrajit S},
  journal={Laryngoscope investigative otolaryngology},
  volume={5},
  number={1},
  pages={96--116},
  year={2020},
  publisher={Wiley Online Library}
}

@article{liu2019roberta,
    title = {RoBERTa: A Robustly Optimized BERT Pretraining Approach},
    author = {Yinhan Liu and Myle Ott and Naman Goyal and Jingfei Du and
              Mandar Joshi and Danqi Chen and Omer Levy and Mike Lewis and
              Luke Zettlemoyer and Veselin Stoyanov},
    journal={arXiv preprint arXiv:1907.11692},
    year = {2019},
}

@article{epstein2010didn,
  title={“I didn’t know what was wrong:” how people with undiagnosed depression recognize, name and explain their distress},
  author={Epstein, Ronald M and Duberstein, Paul R and Feldman, Mitchell D and Rochlen, Aaron B and Bell, Robert A and Kravitz, Richard L and Cipri, Camille and Becker, Jennifer D and Bamonti, Patricia M and Paterniti, Debora A},
  journal={Journal of general internal medicine},
  volume={25},
  pages={954--961},
  year={2010},
  publisher={Springer}
}
Ask

@article{yoshida2015reproducibility,
  title={Reproducibility and diagnostic accuracy of Kellgren-Lawrence grading for osteoarthritis using radiographs and dual-energy X-ray absorptiometry images},
  author={Yoshida, Kanako and Barr, Rebecca J and Galea-Soler, Sandro and Aspden, Richard M and Reid, David M and Gregory, Jennifer S},
  journal={Journal of Clinical Densitometry},
  volume={18},
  number={2},
  pages={239--244},
  year={2015},
  publisher={Elsevier}
}

@article{touvron2023llama,
  title={Llama 2: Open foundation and fine-tuned chat models},
  author={Touvron, Hugo and Martin, Louis and Stone, Kevin and Albert, Peter and Almahairi, Amjad and Babaei, Yasmine and Bashlykov, Nikolay and Batra, Soumya and Bhargava, Prajjwal and Bhosale, Shruti and others},
  journal={arXiv preprint arXiv:2307.09288},
  year={2023}
}


